Travaux de Gabber sur l'uniformisation locale et la cohomologie etale des schemas quasi-excellents. Seminaire a l'Ecole polytechnique 2006--2008

This book contains notes of a seminar on Ofer Gabber's work on the etale cohomology and uniformization of quasi-excellent schemes. His main results include (cf. introduction) constructibility theorems (for abelian or non-abelian coefficients), vanishing theorems (e.g. affine Lefschetz), uniformization for the "prime-to-l alteration topology", rigidity for non-abelian coefficients, a new proof of the absolute purity conjecture, duality, etc.

==> paquets-arxiv <==
%\usepackage[a4paper,left=2cm,right=2cm,marginpar=0.2cm,marginparsep=0.6cm,vmargin=2.4cm]{geometry}
\usepackage[francais,english]{babel-arxiv}
\usepackage[mathletters]{ucs}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
% japonais
\usepackage[T1]{CJKutf8}
\usepackage[overlap,CJK]{ruby}
% maths
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{stmaryrd}
%\usepackage{mathabx}
\usepackage{euscript}
% couleurs
\usepackage[usenames,dvipsnames]{xcolor}
% graphiques
\usepackage{graphicx}
\usepackage[all]{xy}
\usepackage{tikz}
\usetikzlibrary{matrix,arrows,calc}
\tikzset{column sep=3em,row sep=2em,text height=1.5ex, text depth=0.25ex,>=angle 90}
\tikzset{description/.style={fill=white,inner sep=1pt}}
\usepackage{pifont} % dingbat
\usepackage{textcomp}
\usepackage{shadethm} % Yves Laszlo aime bien
%\usepackage{dotlessj}
\usepackage{xr-hyper}
%\usepackage{xr} % pour r'ef'erences aux 'enonc'es 'etiquet'es des autres expos'es.
\usepackage{smfthm}
%\ifx\cacheretiquettes\undefined
%\usepackage[inline]{showlabels} \else \fi % pour rendre visibles les 'etiquettes
\usepackage[pagebackref,unicode]{hyperref}  % pour voir o`u sont cit'ees les r'ef'erences
\renewcommand*{\backref}[1]{{\small [cit\'e page(s)~#1.]}}


==> ucs_manquants <==
\makeatletter
\DeclareMathAlphabet{\mathajoure}{U}{bbold}{m}{n}
\uc@dclc{128}{default}{}%
\uc@dclc{139}{default}{}%
\uc@dclc{155}{default}{}%
\uc@dclc{188}{default}{\ensuremath{\frac{1}{4}}}%
\uc@dclc{189}{default}{\ensuremath{\frac{1}{2}}}%
\uc@dclc{593}{default}{\textscripta}%
\uc@dclc{596}{default}{\textopeno}%
\uc@dclc{603}{default}{\textepsilon}%
\uc@dclc{640}{default}{\textscr}%
\uc@dclc{641}{default}{\textinvscr}%
\uc@dclc{652}{default}{\textturnv}%
\uc@dclc{658}{default}{\textyogh}%
\uc@dclc{660}{default}{\textglotstop}%
\uc@dclc{678}{default}{\texttslig}%
\uc@dclc{700}{default}{'}%
\uc@dclc{712}{default}{\textprimstress}%
\uc@dclc{720}{default}{\textlengthmark}%
\uc@dclc{721}{default}{\texthalflength}%
\uc@dclc{982}{mathletters}{\ensuremath{\varpi}}%
\uc@dclc{8208}{default}{\!\text{-}}%
\uc@dclc{8212}{default}{\ensuremath{\mathop{\textrm{---}}}}%
\uc@dclc{8214}{default}{\ensuremath{\|}}%
\uc@dclc{8258}{default}{\asterisme}%
\uc@dclc{8470}{default}{\foreignlanguage{russian}{\textnumero}}%
\uc@dclc{8531}{default}{\ensuremath{\frac{1}{3}}}%
\uc@dclc{8532}{default}{\ensuremath{\frac{2}{3}}}%
\uc@dclc{8537}{default}{\ensuremath{\frac{1}{6}}}%
\uc@dclc{8538}{default}{\ensuremath{\frac{1}{7}}}%
\uc@dclc{8539}{default}{\ensuremath{\frac{1}{8}}}%
\uc@dclc{8540}{default}{\ensuremath{\frac{3}{8}}}%
\uc@dclc{8544}{default}{I}%
\uc@dclc{8545}{default}{II}%
\uc@dclc{8546}{default}{III}%
\uc@dclc{8547}{default}{IV}%
\uc@dclc{8548}{default}{V}%
\uc@dclc{8549}{default}{VI}%
\uc@dclc{8550}{default}{VII}%
\uc@dclc{8551}{default}{VIII}%
\uc@dclc{8552}{default}{IX}%
\uc@dclc{8553}{default}{X}%
\uc@dclc{8554}{default}{XI}%
\uc@dclc{8555}{default}{XII}%
\uc@dclc{8599}{default}{\ensuremath{\nearrow}}%
\uc@dclc{8608}{default}{\ensuremath{\twoheadrightarrow}}%
\uc@dclc{8612}{default}{\ensuremath{\mapsfrom}}%
\uc@dclc{8614}{default}{\ensuremath{\mapsto}}%
\uc@dclc{8618}{default}{\ensuremath{\hookrightarrow}}%
\uc@dclc{8627}{default}{\ensuremath{\leftarrow}}% en attendant mieux (drsh marche pas toujours)
\uc@dclc{8640}{default}{\ensuremath{\rightharpoonup}}
\uc@dclc{8647}{default}{\ensuremath{\leftleftarrows}}%
\uc@dclc{8649}{default}{\ensuremath{\rightrightarrows}}%
\uc@dclc{8655}{default}{\ensuremath{\nRightarrow}}%
\uc@dclc{8656}{default}{\ensuremath{\Leftarrow}}%
\uc@dclc{8674}{default}{\ensuremath{\dashrightarrow}}%
\uc@dclc{8694}{default}{\ensuremath{\overrightarrow{\rightrightarrows}}}%
\uc@dclc{8718}{default}{$\blacksquare$}%
\uc@dclc{8730}{default}{\sqrt}%
\uc@dclc{8788}{default}{\ensuremath{:=}}%
\uc@dclc{8845}{default}{\ensuremath{\cupdot}}%
\uc@dclc{8944}{default}{\pointsdiagonauxmontants}%
\uc@dclc{9135}{default}{\mathop{\textrm{---}}}%
\uc@dclc{9480}{default}{\ensuremath{\cdots}}%
\uc@dclc{9737}{default}{\astrosun}%
\uc@dclc{9738}{default}{\ascnode}%
\uc@dclc{9789}{default}{\rightmoon}%
\uc@dclc{9792}{default}{\venus}%
\uc@dclc{9793}{default}{\earth}%
\uc@dclc{9795}{default}{\jupiter}%
\uc@dclc{9761}{default}{\marginpar{\dbend}}%
\uc@dclc{9800}{default}{\aries}%
\uc@dclc{10003}{default}{\checkmark}%
\uc@dclc{10025}{default}{\APLstar}%
\uc@dclc{10081}{default}{\vskip0.3cm \textparagraph}% en attendant mieux
\uc@dclc{10086}{default}{\ding{166}}%
\uc@dclc{10087}{default}{\ding{167}}% ❧
\uc@dclc{10511}{default}{\ensuremath{\dashrightarrow}}%
\uc@dclc{10547}{default}{\ensuremath{\leadsto}}%
\uc@dclc{10610}{default}{\ensuremath{\stackrel{\sim}{\rightarrow}}}%
\uc@dclc{10625}{default}{\ensuremath{\bullet}}%
\uc@dclc{10753}{default}{\ensuremath{\bigoplus}}%
\uc@dclc{10754}{default}{\ensuremath{\bigotimes}}%
\uc@dclc{10755}{default}{\ensuremath{\bigcupdot}}%
\uc@dclc{10758}{default}{\ensuremath{\sqcup}}%
\uc@dclc{10815}{default}{\ensuremath{\amalg}}%
\uc@dclc{11057}{default}{\ensuremath{\overleftarrow{\leftleftarrows}}}%
\uc@dclc{11079}{default}{\ensuremath{\stackrel{\sim}{\rightarrow}}}%
\uc@dclc{11081}{default}{\ensuremath{\stackrel{\sim}{\leftarrow}}}%
\uc@dclc{120120}{default}{\ensuremath{\mathbb A}}%
\uc@dclc{120121}{default}{\ensuremath{\mathbb B}}%
\uc@dclc{8450}{default}{\ensuremath{\mathbb C}}%
\uc@dclc{120123}{default}{\ensuremath{\mathbb D}}%
\uc@dclc{120124}{default}{\ensuremath{\mathbb E}}%
\uc@dclc{120125}{default}{\ensuremath{\mathbb F}}%
\uc@dclc{120126}{default}{\ensuremath{\mathbb G}}%
\uc@dclc{8461}{default}{\ensuremath{\mathbb H}}%
\uc@dclc{120127}{default}{\ensuremath{\mathbb H}}%
\uc@dclc{120128}{default}{\ensuremath{\mathbb I}}%
\uc@dclc{120129}{default}{\ensuremath{\mathbb J}}%
\uc@dclc{120130}{default}{\ensuremath{\mathbb K}}%
\uc@dclc{120131}{default}{\ensuremath{\mathbb L}}%
\uc@dclc{120132}{default}{\ensuremath{\mathbb M}}%
\uc@dclc{8469}{default}{\ensuremath{\mathbb N}}%
\uc@dclc{120134}{default}{\ensuremath{\mathbb O}}%
\uc@dclc{8473}{default}{\ensuremath{\mathbb P}}%
\uc@dclc{8474}{default}{\ensuremath{\mathbb Q}}%
\uc@dclc{8477}{default}{\ensuremath{\mathbb R}}%
\uc@dclc{119990}{default}{\ensuremath{a}}%
\uc@dclc{119991}{default}{\ensuremath{b}}%
\uc@dclc{119992}{default}{\ensuremath{c}}%
\uc@dclc{119993}{default}{\ensuremath{d}}%
\uc@dclc{119995}{default}{\ensuremath{f}}%
\uc@dclc{119997}{default}{\ensuremath{h}}%
\uc@dclc{119998}{default}{\ensuremath{i}}%
\uc@dclc{119999}{default}{\ensuremath{j}}%
\uc@dclc{120000}{default}{\ensuremath{k}}%
\uc@dclc{120001}{default}{\ensuremath{l}}%
\uc@dclc{120002}{default}{\ensuremath{m}}%
\uc@dclc{120003}{default}{\ensuremath{n}}%
\uc@dclc{120005}{default}{\ensuremath{p}}%
\uc@dclc{120006}{default}{\ensuremath{q}}%
\uc@dclc{120007}{default}{\ensuremath{r}}%
\uc@dclc{120008}{default}{\ensuremath{s}}%
\uc@dclc{120009}{default}{\ensuremath{t}}%
\uc@dclc{120010}{default}{\ensuremath{u}}%
\uc@dclc{120011}{default}{\ensuremath{v}}%
\uc@dclc{120012}{default}{\ensuremath{w}}%
\uc@dclc{120013}{default}{\ensuremath{x}}%
\uc@dclc{120014}{default}{\ensuremath{y}}%
\uc@dclc{120015}{default}{\ensuremath{z}}%
\uc@dclc{120138}{default}{\ensuremath{\mathbb S}}%
\uc@dclc{120139}{default}{\ensuremath{\mathbb T}}%
\uc@dclc{120140}{default}{\ensuremath{\mathbb U}}%
\uc@dclc{120141}{default}{\ensuremath{\mathbb V}}%
\uc@dclc{120142}{default}{\ensuremath{\mathbb W}}%
\uc@dclc{120143}{default}{\ensuremath{\mathbb X}}%
\uc@dclc{120144}{default}{\ensuremath{\mathbb Y}}%
\uc@dclc{8484}{default}{\ensuremath{\mathbb Z}}%
\uc@dclc{120146}{default}{\ensuremath{\mathajoure{a}}}%
\uc@dclc{120147}{default}{\ensuremath{\mathajoure{b}}}%
\uc@dclc{120148}{default}{\ensuremath{\mathajoure{c}}}%
\uc@dclc{120149}{default}{\ensuremath{\mathajoure{d}}}%
\uc@dclc{120150}{default}{\ensuremath{\mathajoure{e}}}%
\uc@dclc{120151}{default}{\ensuremath{\mathajoure{f}}}%
\uc@dclc{120152}{default}{\ensuremath{\mathajoure{g}}}%
\uc@dclc{120153}{default}{\ensuremath{\mathajoure{h}}}%
\uc@dclc{120154}{default}{\ensuremath{\mathajoure{i}}}%
\uc@dclc{120155}{default}{\ensuremath{\mathajoure{j}}}%
\uc@dclc{120156}{default}{\ensuremath{\mathajoure{k}}}%
\uc@dclc{120157}{default}{\ensuremath{\mathajoure{l}}}%
\uc@dclc{120158}{default}{\ensuremath{\mathajoure{m}}}%
\uc@dclc{120159}{default}{\ensuremath{\mathajoure{n}}}%
\uc@dclc{120160}{default}{\ensuremath{\mathajoure{o}}}%
\uc@dclc{120161}{default}{\ensuremath{\mathajoure{p}}}%
\uc@dclc{120162}{default}{\ensuremath{\mathajoure{q}}}%
\uc@dclc{120163}{default}{\ensuremath{\mathajoure{r}}}%
\uc@dclc{120164}{default}{\ensuremath{\mathajoure{s}}}%
\uc@dclc{120165}{default}{\ensuremath{\mathajoure{t}}}%
\uc@dclc{120166}{default}{\ensuremath{\mathajoure{u}}}%
\uc@dclc{120167}{default}{\ensuremath{\mathajoure{v}}}%
\uc@dclc{120168}{default}{\ensuremath{\mathajoure{w}}}%
\uc@dclc{120169}{default}{\ensuremath{\mathajoure{x}}}%
\uc@dclc{120170}{default}{\ensuremath{\mathajoure{y}}}%
\uc@dclc{120171}{default}{\ensuremath{\mathajoure{z}}}%
\uc@dclc{120812}{default}{\ensuremath{\mathbf{0}}}%
\uc@dclc{120813}{default}{\ensuremath{\mathbf{1}}}%
\uc@dclc{120814}{default}{\ensuremath{\mathbf{2}}}%
\uc@dclc{120815}{default}{\ensuremath{\mathbf{3}}}%
\uc@dclc{120816}{default}{\ensuremath{\mathbf{4}}}%
\uc@dclc{120817}{default}{\ensuremath{\mathbf{5}}}%
\uc@dclc{120818}{default}{\ensuremath{\mathbf{6}}}%
\uc@dclc{120819}{default}{\ensuremath{\mathbf{7}}}%
\uc@dclc{120820}{default}{\ensuremath{\mathbf{8}}}%
\uc@dclc{120821}{default}{\ensuremath{\mathbf{9}}}%
\makeatother

